OSU Multimodal Machine Translation System Report

This paper describes Oregon State University's submissions to the shared WMT'17 task "multimodal translation task I". In this task, all the sentence pairs are image captions in different languages. The key difference between this task and conventional machine translation is that we have corresponding images as additional information for each sentence pair. In this paper, we introduce a simple but effective system which takes an image shared between different languages, feeding it into the both encoding and decoding side. We report our system's performance for English-French and English-German with Flickr30K (in-domain) and MSCOCO (out-of-domain) datasets. Our system achieves the best performance in TER for English-German for MSCOCO dataset.

==> Makefile <==
.PHONY: dvi ps pdf all space clean veryclean distclean

#SHELL = /bin/sh
#MAKE  = gmake

# latex --interaction {batchmode, nonstopmode, scrollmode, errorstopmode}
#TEX = latex --interaction batchmode
TEX = latex 

######################################################################
# source files

texfiles = $(wildcard *.tex)
bibfiles = $(wildcard *.bib *.bst)

tblfiles = $(wildcard tbl/*.tex)

styfiles  = $(wildcard *.sty)

figfiles  = $(wildcard figures/*.fig)
figfiles += $(wildcard figures/*.plt)
figfiles += $(wildcard diagram-*.pdf)
figfiles += $(wildcard figures/*.tex)
figfiles += $(wildcard figures/*.ps)
figfiles += $(wildcard figures/*.epsi)
figfiles += $(wildcard figures/*.c)
figfiles += $(wildcard figs/*.eps)
figfiles += $(wildcard figs/*.gnuplot)
figfiles += $(wildcard figs/*.mp)
#figfiles += $(wildcard figs/*.pdf)
figfiles += $(wildcard figs/*.tex)


figfiles += $(wildcard figures/apps/*.fig)
figfiles += $(wildcard figures/apps/*.plt)
figfiles += $(wildcard figures/apps/*.pdf)
figfiles += $(wildcard figures/apps/*.ps)
figfiles += $(wildcard figures/apps/*.epsi)
figfiles += $(wildcard figures/apps/*.c)

tmp_files = $(wildcard *.log)
tmp_files += $(wildcard *.aux)
tmp_files += $(wildcard *.blg)
tmp_files += $(wildcard *.bbl)
tmp_files += $(wildcard *.toc)
tmp_files += $(wildcard *.dvi)
#tmp_files += (texput.log)

######################################################################
# output files

target =main

######################################################################
# make targets

all:  pdf

simple:
	latex ${target}; dvips -t letter ${target}.dvi -o ${target}.ps


dvi: ${target}.dvi

ps: ${target}.ps

pdf: ${target}.pdf

space:
	@if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	@-/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps

clean veryclean distclean:
	if [ -d fig ]; then cd fig; ${MAKE} $@; fi
	/bin/rm -f ${tmp_files} *~ ${target}.pdf ${target}.ps ${target}.dvi

######################################################################
# rules

%.dvi : %.tex
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	@${TEX} $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		${TEX} $<;	\
		bibtex ${*F};	\
	fi
	@${TEX} $<
#	@-/bin/rm -f ${tmp_files}

%.ps : %.dvi
	dvips -t letter -P pdf -G0 -q -o $@ $<

#%.pdf : %.ps
#	ps2pdf $< $@
#	~/local/macscripts/refresh.scpt

#	cd figs; mptopdf *.mp; cd ..

# %.pdf: %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
# 	pdflatex ${*F} #> ${*F}.log
# 	#tail ${*F}.log
# 	@if  grep Citation ${*F}.log ; then \
# 		bibtex ${*F};   \
# 		pdflatex ${*F};      \
# 		bibtex ${*F};   \
# 		pdflatex ${*F}
# 	#fi
# 	#open $@
# #	~/local/macscripts/refresh.scpt


%.pdf : %.tex ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles}
	@if [ -d fig ]; then cd fig; ${MAKE} all; fi
	pdflatex $<
	@if  grep citation ${*F}.aux ; then \
		bibtex ${*F};	\
		pdflatex $<;	\
		pdflatex $<;	\
	fi
	#@-/bin/rm -f ${tmp_files}
	#pdfcrop --margin "15 15 15 15" main.pdf
	open main.pdf

long.bib:	all.bib
	./remove-short.pl all.bib > long.bib


######################################################################
# dependences

${target}.dvi: ${texfiles} ${bibfiles} ${styfiles} ${figfiles} ${tblfiles} Makefile

